DocTTT: Test-Time Training for Handwritten Document Recognition Using Meta-Auxiliary Learning

Despite recent significant advancements in Handwritten Document Recognition (HDR), the efficient and accurate recognition of text against complex backgrounds, diverse handwriting styles, and varying document layouts remains a practical challenge. Moreover, this issue is seldom addressed in academic research, particularly in scenarios with minimal annotated data available. In this paper, we introduce the DocTTT framework to address these challenges. The key innovation of our approach is that it uses test-time training to adapt the model to each specific input during testing. We propose a novel Meta-Auxiliary learning approach that combines Meta-learning and self-supervised Masked Autoencoder~(MAE). During testing, we adapt the visual representation parameters using a self-supervised MAE loss. During training, we learn the model parameters using a meta-learning framework, so that the model parameters are learned to adapt to a new input effectively. Experimental results show that our proposed method significantly outperforms existing state-of-the-art approaches on benchmark datasets.

==> figures.tex <==
\newcommand{\customfig}[1]{
    \ifnum#1=0
        \setcounter{figure}{0}
        \begin{figure}
            \centering
            \includegraphics[width=1\linewidth]{Weixin Image_20240402212835.png}
            \vspace{-18pt}
            \caption{Illustration of the handwritten document recognition (HDR) problem. Given an input image (left) of a handwritten document, the output of HDR is an XML file (right) describing the page layout. The XML-based representation of the page captures the layout and text tokens of the document image~\cite{albahli2021improved,nurseitov2021handwritten,coquenet2023dan}. The XML representation can be flattened as a sequence of tokens. The goal of our work is to predict this sequence of tokens for a given document image.}
            \label{inputoutput}
        \end{figure}
    \fi
    \ifnum#1=1    
        
        \setcounter{figure}{1}
        \begin{figure*}[htbp]
          \centering
          \begin{tabular}{cccc}
            \textbf{Ground Truth} & \textbf{Masked Image} & \textbf{Reconstructed A} & \textbf{Reconstructed B} \\
            % Row 1
            \begin{subfigure}{0.22\textwidth}
              \includegraphics[width=\linewidth]{sub11.png}
              
            \end{subfigure} &
            \begin{subfigure}{0.22\textwidth}
              \includegraphics[width=\linewidth]{sub12.png}
              
            \end{subfigure} &
            \begin{subfigure}{0.22\textwidth}
              \includegraphics[width=\linewidth]{sub13.png}
              
            \end{subfigure} &
            \begin{subfigure}{0.22\textwidth}
              \includegraphics[width=\linewidth]{sub14.png}
              
            \end{subfigure} \\
            % Row 2
            \begin{subfigure}{0.22\textwidth}
              \includegraphics[width=\linewidth]{sub21.png}
              
            \end{subfigure} &
            \begin{subfigure}{0.22\textwidth}
              \includegraphics[width=\linewidth]{sub22.png}
              
            \end{subfigure} &
            \begin{subfigure}{0.22\textwidth}
              \includegraphics[width=\linewidth]{sub23.png}
              
            \end{subfigure} &
            \begin{subfigure}{0.22\textwidth}
              \includegraphics[width=\linewidth]{sub24.png}
              
            \end{subfigure} \\
            % Row 3
            \begin{subfigure}{0.22\textwidth}
              \includegraphics[width=\linewidth]{sub31.png}
              
            \end{subfigure} &
            \begin{subfigure}{0.22\textwidth}
              \includegraphics[width=\linewidth]{sub32.png}
              
            \end{subfigure} &
            \begin{subfigure}{0.22\textwidth}
              \includegraphics[width=\linewidth]{sub33.png}
              
            \end{subfigure} &
            \begin{subfigure}{0.22\textwidth}
              \includegraphics[width=\linewidth]{sub34.png}
              
            \end{subfigure} \\
            % Row 4
            \begin{subfigure}{0.22\textwidth}
              \includegraphics[width=\linewidth]{sub41.png}
              
            \end{subfigure} &
            \begin{subfigure}{0.22\textwidth}
              \includegraphics[width=\linewidth]{sub42.png}
              
            \end{subfigure} &
            \begin{subfigure}{0.22\textwidth}
              \includegraphics[width=\linewidth]{sub43.png}
              
            \end{subfigure} &
            \begin{subfigure}{0.22\textwidth}
              \includegraphics[width=\linewidth]{sub44.png}
              
            \end{subfigure}
          \end{tabular}
          \caption{Illustration of the handwritten document recognition (HDR) problem across different writing styles with unseen data during testing. The given image consists of four styles (first column), a masked image with 75\% coverage (second column), a reconstruction from low-resolution input (Reconstructed A), and a reconstruction from high-resolution input (Reconstructed B). Predicting the sequence of tokens corresponding to different writing styles from a document image is challenging.}
          \label{fig:my4x4grid} % Assigning a label to the figure
        \end{figure*}
    \fi
    \ifnum#1=2       
        
        \setcounter{figure}{2}
        \begin{figure*}
            \centering
            \includegraphics[width=0.95\linewidth]{2024-06-25 200731.png}
            \vspace{-18pt}
            \caption{Illustration of our model architecture. On the left, the input document image is masked, and encoded into 2D feature maps via a shared FCN Prime encoder. The features of auxiliary encoder are then fed to the self-supervised auxiliary decoder task branch, and the features of the prime encoder are fed to the prime decoder task branch. The auxiliary task branch uses a self-supervised masked autoencoder loss. The primary task branch uses a transformer-based decoder~\cite{coquenet2023dan} architecture to predict the flattened XML representation (see. Figure~\ref{inputoutput}) as a sequence of tokens. }
            \label{Architecture}
        \end{figure*}
    \fi
    \ifnum#1=3       
        
        \setcounter{figure}{3}
        \begin{figure*}
            \centering
            \includegraphics[width=1\linewidth]{2024-06-25 201551.png}
            \vspace{-22pt}
            \caption{Illustration of the Meta-MAE training. For a training example $\mathbf{x_i}$ with ground-truth label $\mathbf{y_i}$, we update the model parameters $\Theta$ using a self-supervised MAE loss (inner loop) to obtain an adapted model $\Theta'$ for this training example. We then use the adapted model $\Theta'$ for the primary task. We then use the supervised loss for the primary task as the meta-objective in the outer loop to update the model parameter $\Theta$.}
            \label{Meta-contrastive training}
        \end{figure*}

    \fi
    \ifnum#1=4   
        
        \setcounter{figure}{4}
        \begin{figure}
            \centering
            \includegraphics[width=1\linewidth]{2024-06-24 021423.png}
            \vspace{-20pt}
           \caption{The auxiliary branch input and output. The input is on the left-hand side and the output is on the right-hand side. In the middle is the Masked image for reconstructing the input image.}
           \label{contrastive learning}
        \end{figure}
    \fi
    \ifnum#1=5    
        \setcounter{figure}{5}
        \begin{figure}[h]
                \centering      \includegraphics[width=0.90\linewidth]{Screenshot 2024-03-25 141510.png} % right figure
                \vspace{-10pt}
                \caption{Sample images from the READ 2016 dataset~\cite{sanchez2016icfhr2016}. The dataset features early modern German scrip. Images are synthetic lines generated with different fronts.}
                \label{fig:read}
        \end{figure}
  
        \setcounter{figure}{6}
        \begin{figure}
            \centering
            \includegraphics[width=1\linewidth]{Screenshot 2024-03-25 133915.png}
            \vspace{-20pt}
            \caption{Sample images from the READ 2016\cite{sanchez2016icfhr2016} dataset: (left) sample image for the single page level; (right) sample image for the double page level.}
            \label{RIMES 2011}
        \end{figure}

        \setcounter{figure}{7}
        \begin{figure}
            \centering
            \includegraphics[width=0.9\linewidth]{Screenshot 2024-03-25 133936.png}
            \vspace{-20pt}
            \caption{Sample images from the Rimes 2011~\cite{grosicki2011icdar} dataset. This dataset contains line-level handwritten sentences.}
            \label{READ 2016}
        \end{figure}
        
        \setcounter{figure}{8}
        \begin{figure}
            \centering
            \includegraphics[width=0.9\linewidth]{2024-07-02 231420.png}
            
            \caption{Sample images from the IAM~\cite{marti2002iam} dataset. This dataset contains paragraph-level handwritten sentences.}
            \label{IAM}
        \end{figure}
    \fi
    \ifnum#1=9
        
        
        \setcounter{figure}{9}
        \begin{figure}
            \centering
            \includegraphics[width=1\linewidth]{Screenshot 2024-04-10 210323.png}
            \vspace{-20pt}
            \caption{Visualization of qualitative examples on the Read 2016 test set. Our DocTTA framework predicts layout entities (shown as a graph on the right) as well as text (written in different colors between each layout entity).}
            \label{qualitative examples1}
        \end{figure}
        \setcounter{figure}{10}
        \begin{figure}
            \centering
            \includegraphics[width=1\linewidth]{2024-06-25 004508.png}
            \vspace{-20pt}
            \caption{Visualization of qualitative examples on four different writing styles. Before and After our DocTTA correct the mistake caused by various handwriting styles during testing.}
            \label{qualitative examples2}
        \end{figure}

}

